What We Can Learn From Visual Artists About Software Development

This paper explores software's role in visual art production by examining how artists use and develop software. We conducted interviews with professional artists who were collaborating with software developers, learning software development, and building and maintaining software. We found artists were motivated to learn software development for intellectual growth and access to technical communities. Artists valued efficient workflows through skilled manual execution and personal software development, but avoided high-level forms of software automation. Artists identified conflicts between their priorities and those of professional developers and computational art communities, which influenced how they used computational aesthetics in their work. These findings contribute to efforts in systems engineering research to integrate end-user programming and creativity support across software and physical media, suggesting opportunities for artists as collaborators. Artists' experiences writing software can guide technical implementations of domain-specific representations, and their experiences in interdisciplinary production can aid inclusive community building around computational tools.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> sections/physical_digital.tex <==
%molly discussing representations between physical and digital
%\begin{quote} So for whatever reason, translating that into a raster image that gets printed on an inkjet printer, feels like a lot of mediation that's not authentic to the work. So I think a lot of it is about finding CNC tools that are a little... They get a little closer to how I'm designing the work. So what I'm coding, and then the physical, the machine production are a little closer aligned. So I think it's part that, and part that I'm really interested in that, the idea that... That digital stuff culturally, the things that are moving as culturally aren't necessarily screen-based. We're very aware of the screen-based stuff, like the Internet, I don't know, music videos, or YouTube. But there are a lot of other things that computing are doing that are making an impact, in a way, say a car is designed, or a college admissions process happens that aren't screen-based.
% \end{quote}



 Furthermore, \aIV, \aX, and \aXI \jingyi{sonia - also others?} all mentioned they liked the ``organic'' and ``warm'' quality of hand drawn art---deviations and irregularities in their artistic style that were built up over learning to draw and physically engaging with their body. These variations are largely absent when working with software programs, and the artists did not consider the task of repetitive manual drawing laborious.

Each participant described a creative workflow involving both digital and manual practice. Facets of artists' non-linear digital-physical practice included enabling and evaluating means of creative expression, encountering challenges in translations from one domain to the other, and engaging embodied knowledge in digital spaces. 

Power of software- working across media/ output: Michael described technology as exposing the ability to work across mediums to create something that can be perceived as "a drawing and a sculpture and an animation, all the same."
% -- Enabling creative expression 

% Generating imagery 
To begin with how artists integrate digital and physical affordances to enable creative expression, Emily, Nina, and Fish moved between physical and computational tools to generate imagery. For instance, Emily described using digital photography or scanning to create textures and "incorporate as many non-computer elements into the digital artwork" while Fish discussed slicing drawings by photographing physical artifacts and reconstructing them digitally "like print-makers." Nina described scanning, tracing, digitizing sketches over copies of architectural plans and how she uses scanning and copying tools as "just a mechanism to do something with imagery."

% Convergence of an artifact that is either computational or physical through an integrated digital and physical workflow 
Artists also use the process of moving between computational and digital domains as a way to develop creative pathways to refine artifacts. Moreover, these artifacts can be either digital or physical. Chris described "making tools as the sort of, post-birthing process of art." Ben and Kim depicted painting. Ben discussed his process for considering how the materiality of paint shapes his work in converging a digital representation and physical artifact. Kim described prototyping with physical painting while relying on "huge libraries of images and washes, the textures." Fish portrayed how he advocates for refining a drawing through cyclical physical and digital manipulation. He claims it makes work that is "markedly better and it looks more human." He shared: 
\begin{quote}
    \textit{Why don't you put a piece of tracing paper over the screen right now, and just physically draw it? And then let's look at the drawing. And then let's open up Illustrator, and then create a version of it again.}
\end{quote}

% Collaboration based on evaluating both physical artifacts and ways of working enabled by custom computational tools
Collaborative workflows between artists focused on manual practice versus tool building rest on moving between the two domains to the point of integrating them in order to evaluate creative possibilities afforded by custom computational tools. Emily and Michael, who both take on the role of the artist primarily using tools created by their collaborators, shared that this process involves evaluating both physical artifacts and ways of working enabled by custom computational tools. Emily described drawing with tools that she composited into a character and their process for interweaving hand-drawing with tool development. In addition to being a back and forth between collaborators, the process is a back and forth between manual and procedural work. The example Michael shares differs in that the manipulation of the artifact is more physical than digital. Michael used the outputs enabled by Chris's tools to "manually rip it apart and start to draw with it," and because Michael draws with the tools shared by Chris, Michael considers Chris' code as drawing. 

% -- Encountering challenges

%  Challenges in translating between physical to digital and digital to physical practice  
In addition to depicting how non-linear workflows between digital and physical spaces lead to avenues for creative expression, artists described challenges in moving from one domain to the other. On on hand, when moving from physical to digital representations, Mac described making low level edits to digital artifacts to manipulate distinct, undesirable visual properties such as "crisp" svg files. Emily, who replicated her drawing and notes such as a character and ideas for its movement in multiple mediums, described digitizing sketches as unnecessarily laborious and repetitive. On the other hand, in moving from digital to physical artifacts, artists discusses the need for physical feedback and interaction in order to iterate on artwork. Miwa and Emily both noted the challenge of designing on a screen to project large-scale animations and needing to revise computational designs based on the full-scale experience of their work. Kim mentioned how she frames scale in relation to her body and finds that process to be challenging in a digital setting. Nina shared she likes "going back and forth" because it's necessary for her to have the "tangible" experience "to literally put stuff down on the floor and look at it." Both Lynn and Nina elaborated how "proportions and visual relationships" need to be assess physically because balance and weight are perceived differently on a screen.  

% -- Engaging embodied knowledge digitally 

% Divided opinion on whether sketching is tactile digitally
\sonia{I'm not sure if this point belongs in this section / if this is framed correctly}
While artists visual creative work spanned engaging in manual and computational practice, artists contrasted the tactility of sketching in a physical versus digital setting. Emily, Fish and Lynn specifically described starting on paper for "sketching or writing," "to warm up," or "because it's a little more fluid," respectively. Michael, however, stated "drawing on a computer is just as fun and tactile as doing it with charcoal, really." Shantell shared her experience of how drawing in VR allowed her to work in a digital and physical domain simultaneously. With respect to her practice, she elaborated: 
\begin{quote}
    \textit{my medium is drawing and that can be applied in the function of high or low tech.... I basically say I draw just to simplify things and then medium and the application can change.}
\end{quote}

% Relating digital workflows to physical production to create an integrated practice (does this go here??) / how can this be recast?
Artists also related digital workflows to physical production. Nina elaborated on how practice has helped her map visual relationships in a digital space to a physical environment and how the visual creative process is the same in either domain. Ben shared how knowledge of a computational tool can be "tactile, physical and potentially even emotional." He spoke of "operating machines in ways that are extensions, not only of your hand, but of your mind." Fish compared and equated the incremental process of coding to drawing. 

% Working out computational ideas through physical production 
Lastly, Emily and Molly provided specific examples of working out computational ideas through physical production. Emily came up with the ideas for an computational rules to define an interactive generative puzzle game while working on a hand-sketched maze. Molly shared how her domain knowledge in physical production and manual practice helps her work out computational ideas:
\begin{quote}
\textit{I've been switching back and forth between doing a little coding and doing a little felting or folding. And a lot of times, I will solve my code problems while I'm felting in my head}
\end{quote}

In sum, artists demonstrated finding opportunities for creative expression through non-linear workflows spanning digital and physical domains, facing challenges beyond representation in working across physical and digital spaces, and leveraging embodied knowledge from physical production into an  integrated physical and digital practice.








==> sections/tools_artwork.tex <==
Reasons artists were drawn to tools included testing new concepts, evaluating interaction design, contributing to communities, accessing flow, and adding organic overtures~\jj{organic overtures is unclear.} to work~\jj{this sentence is much clearer than the previous two.- maybe just make this the introduction to this section? Let's try to avoid passive voice though. Also, let's order the introduction in the order we talk about things in the rest of the section}. 

% Tools as a means to enact constraints - artists code it into the tool / choose tools based on those constraints  (e.g. Michael) -- deliberately author or choose an exsiting piece of software 
Perhaps unsurprisingly~\jj{is this unsurprising?}, several artists described computational tools as digital pencils and making tools as an opportunity to delve into either a concept or means of execution~\jj{not clear how the digital pencils part is connected to rest of this sentence}. Ben stated "if you only had triangular brushes, if you look in the world you would only see triangles."~\jj{not sure how strong this quote is. @Jingyi what are your thoughts?} Fish too underscored the ability to deepen conceptual knowledge when working with a specific tool. Six artists stressed that tools can be used as mechanisms to test ideas and specifically refer to ideas for way of working. Eran, Kim, and Michael in particular discussed engaging creativity through constraint-based tools to prompt visual discovery. For instance, Eran described creating conditional constraints on color picking: 
\begin{quote}
    \textit{you know, like every, every stroke we put on the canvas shifts the hue, like in a very very tiny, tiny, tiny difference. Every stroke. And then every 14th stroke is a complementary color and then it goes back. And just trying these things, you know, it's like a, maybe, it's kind of like the John Cage kind of thinking}
\end{quote}~\jj{I like this section but we need to be cautious to differentiate it from the learning program as a means of investigating creative possibilities part of the motivations section}
% 6 artists = Michael, Eran, Kim, Michael, Lynn and Emily

% Tools to manipulate artwork to explore expressive possibilities (inverse of constraint sections) -- select existing tool or create new software 
% To enact constraints & specific forms of freedom / expression by selection or coding their own. Deliberate about ways of being controlled or creating control 
Next, multiple participants depicted tool building to explore interaction design.~\jj{ I like these examples, but i don't think interaction design is the right term for this. Also michael's example isn't about tool building} Chris framed technology as affording participatory artwork. Michael described technology as exposing the ability to work across mediums to create something that can be perceived as "a drawing and a sculpture and an animation, all the same." \sonia{add to phys/digital} Eran focuses on the question, "how will it feel?" He focused on the experience of controlling a character via a synthesizer. Mac discussed coding to create a means to support dynamic navigation in digital comics. Finally, moving collages, at the core of Miwa's work, were enabled through the use of computational tools as she began by using flash to animate collages set to music. She mentioned implementing visual illusions through projection, digital collage, and motion graphics to communicate casual relationships: 
\begin{quote}
    \textit{you’re working with a ephemeral media, which is light. There’s ways to make it look like it can touch each other and react to each other and have consequence to each other, which is through choreography and storytelling and performance}
\end{quote}~\jj{I like Miwa's example, but is it about tool building? How are we defining tool building in this section?}

% Talk more about Emily's example (organic patina) 
Lastly, artists described tool building and use~\jj{why are we conflating tool building and tool use?} to support alternative forms of engagement~\jj{alternative forms of engagement is vague. can we be more descriptive here?}. For instance, 4 artists discussed a preference to use task-specific tools that add character in opposition to general purpose tools. Nina added that a worthwhile tool leads to personal output and Michael shared realizing his ability to "dissolve the lines between what tools were 'meant for what purposes.'"~\jj{quote wording unclear...} 
Lynn, Emily, and Eran shared using personal inputs that leave an organic patina on work. This ranged from Lynn describing making a font based on her cat walking to Emily illustrating both visualizing audio data and, in partnership with her collaborators Nick and Theo, leveraging custom tools to add manual, descriptive elements to programmatic behavior so "it still feels like real animation and not programmed animation." In reference to one particular project, she reflects on their process: 
\begin{quote}
    \textit{can the plant just do this? Can it do this? And then they ended up building these whole kind of editors and they're amazing tools that gave me so much more control over how something moves}
\end{quote}~\jj{have to describe what plant is? give context}

% Ad hoc tools, Emily / Theo posters  
Moreover, artists' alternative approaches towards computational tools were manifest~\jj{simpler term? present? also, avoid passive voice.} in their notions surrounding presentation and use. Chris demarcates~\jj{use plainer language, ``described''?} his software as "plug-ins" in opposition to tools and contrasted "a little input box" to creating a "plug-in" that could be used to create specific, artist-driven variation. Eran expounds~\jj{plain language. ok to repeat the same term.} on not making "bullet-proof tools" as opposed to "small prototypes." Lastly, Emily describes tool release~\jj{does this mean releasing tools to other people? clarify.} as collaborative storytelling.

% Tools are the art 
First, in developing software to create tools, 4 artists described how the tool itself becomes the artifact. Kim added focusing on the conversation precipitated by the act of developing a particular tool. She stated "I don't see it as a tool or I see it more as an art project in and of itself."~\jj{this quote is unclear out of context. can we just describe what she meant? I think we only need one quote per example at most, so we should pick the ones that are easiest to understand as standalone fragments.} Chris too stated "I saw those pieces of software as the artwork." Molly elaborated that, as tool making represents problem-solving for repeated use in work, it becomes intrinsic to her artistic interpretation and compared the notion to sculptors in studio practice designing their own chisels.~\jj{wordy sentence. simplify and clarify and possibly break into two sentences. Also does this overlap with the next section?}

% Get rid of this / use as summary or conclusion 
Artists motivated either making specific choices around tools or choosing to build custom computational tools to make artwork as ways to engage concepts that facilitate expressiveness, to examine  possibilities that are afforded by multimedia, and to support divergent forms of engagement that mitigate imposed digital aesthetics and lower floors. ~\jj{should this (and the following be a separate section?}~\jj{emily discussed heavily here? justify?}

\sonia{where does this go?}
Chris and Eran described tool building to support communities. Chris illustrated wanting to lower the floor for creatives to use technology either without having to program explicitly to develop wearables or to use layers as a primary abstraction in VR. 

\sonia{where does this go?}
Distribution constraints. Lynn's lowest common denominator font renderers

\jj{closing summary needed.}

% Ways to rely on tools
% Delve into concepts 
% Polish / tune work 

% Ways artists leverage tools can impose constraints

% Ways artists enable new expressive possibilities or degrees of freedom 







